Comprehensive multi-wavelength modelling of the afterglow of GRB050525A

The Swift era has posed a challenge to the standard blast-wave model of Gamma Ray Burst (GRB) afterglows. The key observational features expected within the model are rarely observed, such as the achromatic steepening (`jet-break') of the light curves. The observed afterglow light curves showcase additional complex features requiring modifications within the standard model. Here we present optical/NIR observations, millimeter upper limits and comprehensive broadband modelling of the afterglow of the bright GRB 0505025A, detected by Swift. This afterglow cannot be explained by the simplistic form of the standard blast-wave model. We attempt modelling the multi-wavelength light curves using (i) a forward-reverse shock model, (ii) a two-component outflow model and (iii) blast-wave model with a wind termination shock. The forward-reverse shock model cannot explain the evolution of the afterglow. The two component model is able to explain the average behaviour of the afterglow very well but cannot reproduce the fluctuations in the early X-ray light curve. The wind termination shock model reproduces the early light curves well but deviates from the global behaviour of the late-time afterglow.

==> Table_Jbandhost_photometry.tex <==
\begin{table*}
\caption{$J$-band astrometry and photometry of sources located close to the {\it Swift} XRT error circle}
\centering
\smallskip
\begin{tabular}{c c c c c}
\hline \hline
Source &  RA          & Dec          &  Magnitude    & err \\ 
       &  (J2000)     & (J2000)      &   (mag)       & (mag) \\  
\hline
1      & 18:32:32.759 & +26:20:20.06 & 23.304      & 0.208\\
2      & 18:32:32.593 & +26:20:20.86 & 23.581      & 0.225\\
3      & 18:32:32.422 & +26:20:20.32 & 23.252      & 0.208\\
4      & 18:32:32.255 & +26:20:20.78 & 24.086      & 0.422\\
\hline                                   
\end{tabular}
%\newline
%$^\dagger$ Burst trigger time: 2005 May 25.002 d\\
\label{table3}      
\end{table*}


==> Table_host_observations_log.tex <==
\begin{table*}
\caption{Log of host galaxy observations}
\centering
\smallskip
\begin{tabular}{c c c c c l}
\hline \hline
Date-obs (UT)             & Time since burst ($T$)$^\dagger$ & Magnitude    & Exp time        &  Filter & Telescope\\
 (d)                      &    (d)                     & (mag)        &  (s)            &         &          \\
\hline
2011-05-26.1508--30.0955  & 2131.1488--2135.0935       &  $<$24.1               & 18$\times$900   &  g      & 2.2m-CAHA\\
2011-05-26.1508--30.0955  & 2131.1488--2135.0935       &  $<$24.3               & 18$\times$900   &  r      & 2.2m-CAHA\\
2011-05-28.9855--30.0955  & 2133.9845--2135.0935       & 25.1$\pm$0.4           & 17$\times$900   &  i      & 2.2m-CAHA\\
2011-07-18.0320--18.1150  & 2245.0301--2245.1131       & 23.58$\pm$0.225$^{\dagger\dagger}$ & 83$\times$60    &  J      & 3.5m CAHA\\
2011-07-19.0502--19.1077  & 2246.0483--2246.1059       &    --                              & 57$\times$60    &  J      & 3.5m CAHA\\
\hline                                   
\end{tabular}
\newline
$^\dagger$ $T=t-t_0$ where $t_0=$25-05-25.002 d

$^{\dagger\dagger}${The magnitude is the result of the combination of the J-band data taken on 18 and 19 July 2011.}
\label{table4}      
\end{table*}

